MotionCanvas: Cinematic Shot Design with Controllable Image-to-Video Generation

This paper presents a method that allows users to design cinematic video shots in the context of image-to-video generation. Shot design, a critical aspect of filmmaking, involves meticulously planning both camera movements and object motions in a scene. However, enabling intuitive shot design in modern image-to-video generation systems presents two main challenges: first, effectively capturing user intentions on the motion design, where both camera movements and scene-space object motions must be specified jointly; and second, representing motion information that can be effectively utilized by a video diffusion model to synthesize the image animations. To address these challenges, we introduce MotionCanvas, a method that integrates user-driven controls into image-to-video (I2V) generation models, allowing users to control both object and camera motions in a scene-aware manner. By connecting insights from classical computer graphics and contemporary video generation techniques, we demonstrate the ability to achieve 3D-aware motion control in I2V synthesis without requiring costly 3D-related training data. MotionCanvas enables users to intuitively depict scene-space motion intentions, and translates them into spatiotemporal motion-conditioning signals for video diffusion models. We demonstrate the effectiveness of our method on a wide range of real-world image content and shot-design scenarios, highlighting its potential to enhance the creative workflows in digital content creation and adapt to various image and video editing applications.

==> Sections/sec-1-intro-old.tex <==


\section{Introduction}
\label{sec-1-intro}

Image animation, also known as image-to-video generation (I2V), offers a powerful tool for video creation, allowing filmmakers and content creators 
to bring static images to life with dynamic motion. 
Over the years, image animation has attracted significant research efforts~\cite{horrytour, xuanimating,niklaus3d,liuinfinite, holynski2021animating}, exploring various approaches to animate still images.
Recent advances in modern video generation models have transformed the landscape of I2V 
%image-to-video 
synthesis~\cite{xing2023dynamicrafter,yang2024cogvideox}. These models utilize generative techniques 
%modeling techniques to generate 
to produce videos from textual descriptions, opening up new creative possibilities. However, the limitations of pure I2V approaches become clear when considering the complexities of dynamic content, as textual information alone often falls short of 
%fails to 
capturing the intricate details of the motion, leading to uncertainty and a lack of control in generating the animations.

In content creation and filmmaking, motion design of the shot is crucial. It involves planning the camera movements and object motions to create a cohesive visual narrative. Despite its importance, current video generation models \phil{rely primarily} on textual input\phil{s} for motion control, which \phil{largely} limits the precision and expressiveness of the resulting animations. \phil{Some?} Existing works \phil{cite some here?} attempt to incorporate camera and object motion controls in video diffusion models.
However, they \phil{cannot fully address} 
%have not fully addressed 
the challenges of shot design.
%Specifically, they face two main limitations: the lack of joint modeling for camera and object motions, and the absence of 3D-aware motion conditioning signals.
\phil{Specifically, the challenges come from (i)} the lack of joint modeling for camera and object motions, and (ii) the absence of 3D-aware motion conditioning signals.

\phil{TO NOTE: it will be good to explain the paper title here (or revise the title), e.g. interactive? Does this work support interactive?}

\phil{The next sentence is important. Make sure the sentence clearly describes this work without overly claiming something or misleading, e.g., did you relate camera movements with object motion?}
To define our problem, we focus on the relationship between camera movement and scene-aware object motion within the temporal range of a shot. This involves representing each motion signal in a way that accurately reflects user intentions while remaining suitable for training video generation models. The key challenges include the following:

\textbf{Designing Control Signals}: Creating control signals that effectively communicate \phil{describe? model? capture?} user intentions for both camera and object motions.

\textbf{Generating Video with User Intentions}: Ensuring that the generated video aligns with the specified motion intentions.

\textbf{Separating Camera and Object Motion}: Distinguishing between camera movements and object motions to achieve coherent animations \phil{natural video generation?}.

Our findings indicate that, while users think about motion in scene space, models are often trained more effectively with screen-space signals. We propose that the first frame of the video can serve as a canvas for users to express their scene-space motion design intent. Additionally, classical graphics and 3D vision techniques offer natural methods for separately representing object positioning and camera movements.

To address these challenges, we introduce \MOCA, a streamlined video synthesis system designed for cinematic shot design. Our method enables comprehensive motion control, allowing for the joint manipulation of both camera and object motions in a scene-aware manner during the shot design and video synthesis processes. We develop dedicated motion-conditioning mechanisms that guide DiT-based video diffusion models to follow control signals capturing camera and object motions. Coupled with a Motion Signal Translation module, our approach translates depicted scene-space motion intent into screen-space conditioning signals for the video generation module.

In summary, this paper makes the following contributions.

\begin{itemize} 
%
%\item We introduce the problem of cinematic shot design in image-to-video synthesis. 
\item We introduce cinematic shot design to the process of image-to-video synthesis. 
%
\item We present \MOCA, a streamlined video synthesis system for cinematic shot design, 
%enabling 
\phil{offering} holistic motion control\phil{s} 
%that allows 
for joint manipulation of camera and object motions in a scene-aware manner. 
%
\item 
%To this end, 
Further, we design dedicated motion conditioning mechanisms to guide the DiT-based video diffusion models with 
%in following 
the control signals that capture the camera and object motions. We couple that with a Motion Signal Translation module to translate the depicted scene-space motion intent into the screen-space conditioning signal for the Video Generation module. 
%
\item Evaluations on diverse 
%range of 
real-world photos 
%input images 
demonstrate the effectiveness of \MOCA for cinematic shot design, highlighting its flexibility and potential for various creative applications. 
%
\end{itemize}


==> Sections/sec-1-intro-tt.tex <==


\section{Introduction}
\label{sec-1-intro}

{\bf [TT version:]} Image animation, also known as image-to-video generation (I2V), offers a powerful tool for video creation, allowing filmmakers and content creators 
to bring static images to life with dynamic motion. 
Over the years, image animation has attracted significant research efforts~\cite{horrytour, xuanimating,niklaus3d,liuinfinite, holynski2021animating}, exploring various approaches to animate still images.
Recent advances in modern video generation models have transformed the landscape of I2V 
%image-to-video 
synthesis~\cite{xing2023dynamicrafter,yang2024cogvideox}. These models utilize generative techniques 
%modeling techniques to generate 
to produce videos from textual descriptions, opening up new creative possibilities. However, the limitations of pure I2V approaches become clear when considering the user-intent dynamic content, as textual information alone falls short of 
%fails to 
capturing the intricate details of the motion, leading to uncertainty and a lack of control in generating the animations.

In content creation and filmmaking, motion design of the shot is crucial. It involves planning the camera movements and object motions to create a cohesive visual narrative. Despite its importance, current video generation models rely primarily on textual inputs for motion control, which largely limits the precision and expressiveness of the resulting animations. Some existing works~\cite{wang2024motionctrl,wu2025draganything} attempt to incorporate camera and object motion controls in video diffusion models.
However, they cannot fully address the challenges come from the intertwining nature of camera and object motions, and hence struggle to interpret the ambiguous user intention. For instance, when user drags the arm of a character in the image, it could mean panning the camera, moving the character, or just moving the arm. 

In our work, we aim at enabling the precise user control of camera motion, object global motion (moving the character), and object local motion (moving the arm). 
A straightforward approach is to prepare video training data owning all required labels (e.g. camera extrinsic parameters, object motion, etc). 
But this requires labor-intensive and possibly unreliable labeling, and eventually limits the variety and quantity of video data for training~\cite{wang2024motionctrl,he2024cameractrl}. 
Instead, we propose to represent motions that do not rely on such intensive labels, but on simple 2D bounding boxes and 2D point trajectories that can be automatically and reliably estimated. 
This allows us to take almost any kind of videos for training, and enriches our generation variety.

However, we still have one major problem left. 
Users tend to think and plan the motion in 3D scene space, but the video generation model is trained in 2D screen space. 
Moreover, users have to specify the motion plan on the 2D image canvas. 
In other words, we need an effective translation from the user motion plan in 3D scene space to control signals (bounding boxes and point trajectories) in 2D screen space. 
Based on the classical scene modeling in computer graphics, we propose the motion signal translation module that allows users to plan motion in 3D scene space, and then accurately interpret the user intention. 
This module can decompose the user motion into hierarchical transformation and rectify the potentially erroneous user input before feeding the interpreted 2D control signals to the video generation model.



%Specifically, they face two main limitations: the lack of joint modeling for camera and object motions, and the absence of 3D-aware motion conditioning signals.
%\phil{Specifically, the challenges come from (i)} the lack of joint modeling for camera and object motions, and (ii) the absence of 3D-aware motion conditioning signals.

%\phil{The next sentence is important. Make sure the sentence clearly describes this work without overly claiming something or misleading, e.g., did you relate camera movements with object motion?}
%To define our problem, we focus on the relationship between camera movement and scene-aware object motion within the temporal range of a shot. This involves representing each motion signal in a way that accurately reflects user intentions while remaining suitable for training video generation models. The key challenges include the following:

%\textbf{Designing Control Signals}: Creating control signals that effectively communicate \phil{describe? model? capture?} user intentions for both camera and object motions.

%\textbf{Generating Video with User Intentions}: Ensuring that the generated video aligns with the specified motion intentions.

%\textbf{Separating Camera and Object Motion}: Distinguishing between camera movements and object motions to achieve coherent animations \phil{natural video generation?}.

We called our streamlined video synthesis system \MOCA,
allowing for the joint manipulation of both camera and object motions in a scene-aware manner during the shot design and video synthesis processes. 
We develop dedicated motion-conditioning mechanisms that guide DiT-based~\cite{peebles2023scalable} video diffusion models to follow control signals capturing camera and object motions. 
In summary, this paper makes the following contributions.

\begin{itemize} 
%
%\item We introduce the problem of cinematic shot design in image-to-video synthesis. 
\item We introduce cinematic shot design to the process of image-to-video synthesis. 
%
\item We present \MOCA, a streamlined video synthesis system for cinematic shot design, 
%enabling 
\phil{offering} holistic motion control\phil{s} 
%that allows 
for joint manipulation of camera and object motions in a scene-aware manner. 
%
\item 
%To this end, 
Further, we design dedicated motion conditioning mechanisms to guide the DiT-based video diffusion models with 
%in following 
the control signals that capture the camera and object motions. We couple that with a Motion Signal Translation module to translate the depicted scene-space motion intent into the screen-space conditioning signal for the Video Generation module. 
%
\item Evaluations on diverse 
%range of 
real-world photos 
%input images 
demonstrate the effectiveness of \MOCA for cinematic shot design, highlighting its flexibility and potential for various creative applications. 
%
\end{itemize}


==> Sections/sec-3-method-long.tex <==

\section{\MOCA}
\label{sec-3-method}

%%%%%%% Figure: Overall Pipeline %%%%%%%
\input{Figures/fig-overall-pipeline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% [Motivate our method design: capturing user motion design intention, and generate videos respecting such design.]
% [Describe the overview of our method: our overall pipeline consists of 3 main components. Motion Design module, Motion Signal Translation module, Video Synthesis module.]
% [Briefly summarize each component.]
Our method animates still images into short videos reflecting the user's motion design intentions. As illustrated in Fig.~\ref{fig:overall-pipeline}, the proposed approach comprises three main components: (1) a motion design module capturing diverse scene-aware motion intentions, (2) a translation module converting these intentions into screen-space motion signals, and (3) a motion-conditioned video generation model. 

% [Refer to figure \ref{fig:overall-pipeline}]

\subsection{Motion Design Module -- Capturing User Intents}
\label{sec-3.1-motion-design}
% [Discuss the principles of \MOCA: depicting motion in scene space, with the first frame establishing the frame of reference.]
% [We enable a unified interface to control camera motion, object global motion, object local motion, and timing.]
We leverage the input image as the canvas for motion design, establishing a starting scene on which the motion designs are grounded. This enables 3D-scene awareness in the motion design process, capturing spatial relationships between objects, the camera, and the scene. Our unified interface facilitates individual control over camera motion, object global and local motion, and their timing.

\textbf{Camera Motion Control with 3D Camera Paths.}
% [Discuss how camera motion information is defined]
% [Describe how camera motion is specified by users and how parameters are calculated]
We define camera motion using standard pinhole camera parameters, specifying a 3D camera path, $P$, as a sequence of extrinsic $E_l$ and intrinsic $K_l$ parameters for each frame $l$: $(E_l, K_l)_{l=1}^{L}$, where $E_l\in \mathbb{R}^{3\times4}$ and $K_l \in \mathbb{R}^{3\times 3}$.
To design the camera path, users can specify the camera poses (\textit{i.e.} the translation vector and rotation angles with respect to the initial view) at key moments. The full camera path can be obtained via interpolation.
To make the camera path specification process more intuitive for users, our system also lets users specify and mix $M$ base motion patterns (\textit{e.g.}, panning, trucking, dolly) along with the corresponding direction and speed. Our method then converts the user-specified camera motion patterns into the corresponding 3D camera paths. 

%$(E_l^{(m)}, K_l^{(m)})$ and combines them into the overall camera path $E_l=\prod_{m=1}^M E_l^{(m)}$, $K_l$ is an average across $K_l^{(m)}$'s assuming normalization to the first frame. 

\textbf{Object Global Motion Ctrl. with Scene-Anchored Bounding-Boxes.}
% [Discuss the importance of global object motion control in shot design]
% [Discuss how the location in the scenes that the object traversing can be depicted with bounding boxes: position and size.]
Controlling where the objects move within the scene is crucial in designing video shots. 
We argue that such global object control should be defined in a scene-aware manner in which object positioning is grounded to positions in the underlying 3D scenes.
To this end, we enable users to perform scene-aware bounding boxes (bboxes) placement by minimally specifying start and end points, as well as (optionally) intermediate key points. 
By anchoring the bbox placements to the fixed view established by the input image, users can depict the imagined target locations via adjusting not only the position but also the scale and shape of the boxes. This scene-aware bbox placement provides intuitive control over object position, scale, pose, and relative distance to the camera.
From the provided key bbox positions and intended duration of the output video, we generate smooth box trajectories via Catmull-Rom spline interpolation~\cite{catmull1974class}. 

\textbf{Object Local Motion Control with Point Tracing.}
% [Define local object motion]
% [Discuss the scenarios where local object motion control is desirable]
% [Describe our method to depict local object motion control]
While global object motion defines how objects change their position within the scene and is our main focus in the shot design process, local object motion -- depicting in-location movement of objects (\textit{e.g.}, raising arms, a rotating head) -- can also enrich the shot design experience with added details and realism.
Inspired by the recent success of drag-based editing~\cite{wu2025draganything,mou2024revideo}, we use sparse point trajectories to depict local motions. As local motion often involves complex geometric relationships and deformations, sparse point trajectories offer a flexible way to define and manipulate such motions.

\textbf{Timing Control}.
% [Discuss the importance of timing control]
% [Emphasize that our method enables natural way to control timing: assign the timeline along the camera and object motion trajectory.]
%Timing control determines the pace and emotional impact of a scene. Precise timing ensures that object and camera motions align seamlessly, enhancing narrative flow and visual coherence.
%Our method enables a natural way to control timing by allowing users to assign a timeline directly along the camera and object motion trajectories, ensuring smooth and intuitive adjustments to the temporal dynamics of a scene.
Timing control of the object and camera motions allows them to be designed in a coordinated manner, enhancing narrative flow and visual coherence. Our system naturally supports timing control by letting users assign a timeline directly along the motion trajectories.

\subsection{Motion Signal Translation Module}
% [Recall the key insight: motion intent is best developed in scene space, but video generation models are better trained in screen space.]
% [Discuss the type of screen-space conditioning signals that has been shown promising. Motivate our key idea: converting scene-space motion design to spatiotemporally grounded screen-space control signals.]

While motion intent is best designed in the 3D-aware scene-centric manner, video generation models are often most effectively trained for motion conditioning with 2D screen-space, frame-centric data in which all motion types have been mixed together after view-dependent projections. 
This discrepancy arises due to the challenging nature of extracting reliable 3D information such as camera motions and 3D object trackings in general videos at large scales~\cite{zhou2018stereo}. 
To address this challenge, instead of aiming to devise a video generation model that directly handles the designed scene-space motion information, our key idea is to translate the scene-space motion design obtained from Section~\ref{sec-3.1-motion-design} into the spatio-temporally grounded screen-space motion signals that can be reliably extracted from in-the-wild videos. 

\paragraph{\textbf{Camera Movement via Point Tracking}}
% [Motivate why point tracking is a good representation to control camera movement]
% [Discuss the advantages of using point tracking to control camera motion: flexible dense and sparse controls, robust to extract from real videos]
% [Describe the details of how 3D camera trajectories are converted to point tracks]
We seek a form of screen-space motion signal that (1) can be robustly extracted from general video data, and (2) encodes detailed information about the camera movement throughout the videos.
Research on human visual perception~\cite{perception book} offers the important insight that egocentric motion can be reliably recovered by a sparse set of scene point trackings projected onto the image plane. This insight has been widely applied in classical computer vision methods for camera pose estimation~\cite{survey paper}, structure from motion~\cite{survey paper}, and SLAM~\cite{survey paper}.
Inspired by this insight, we represent camera movement using point tracking. We note that this information can be robustly extracted from real videos~\cite{cho2025local,karaev2024cotracker3}. 

At inference time, we convert 3D camera paths to 2D point tracks by randomly sample a set of points on the input image. To focus on points belonging to static background, which better reflect the camera movement, we exclude regions from likely-moving objects estimated from a YOLOv11~\cite{khanam2024yolov11}-generated mask. 
We then use an off-the-shelf monocular depth estimator~\cite{wang2024moge} to obtain intrinsic camera parameters and a depth map. Finally, we warp these points based on the 3D camera path and depth, creating corresponding 2D screen-space point tracks.

\paragraph{\textbf{Scene-aware Object Motion via Bounding-box Trajectories}}
%\paragraph{\textbf{From Scene-Centric Object BBox Placements to Frame-Centric Bbox Trajectories}}
% [Re-emphasize the difference between the bounding box trajectories specified by the users and the screen-space information that can be extracted from real videos. Motivate the need to convert from scene-space to screen-space box trajectories.]
% [Describe our technique for box trajectory conversion.]
User-defined scene-space bbox trajectories reflect motion intent but are distorted by camera movement and perspective when projected onto the screen. 
We aim to convert such scene-anchored object bboxes to screen space in a way that resembles the object bbox sequence typically extracted from real videos. 
We first lift the scene-space bbox to 2.5D, using camera pose and depth to continuously reproject it into screen space across frames. The initial bbox's depth is the average depth within its SAM2~\cite{ravi2024sam}-generated semantic mask. Subsequent bboxes use either (1) a reference depth from a point in the scene (e.g., the ground plane) or (2) a depth based on perspective consistency, where a bbox growing in size implies movement toward the camera.
Using the assigned depth and camera pose transformations, the 2.5D bboxes $b_\text{scene}^l$ at time $l$ are projected into screen space $b_\text{screen}^l$ with calibrated locations and sizes:
\begin{equation}
    b_\text{screen}^l = \mathcal{T}_\text{camera}^l(b_\text{scene}^l),
\end{equation}
where $\mathcal{T}_\text{camera}^l(\cdot)$ denotes the camera motion transformation.


\paragraph{\textbf{Object Local Motion via Point Trajectory Decomposition}}
% [Motivate the need to control fine-grained object motion.]
% [Formally define the local object motion.]
% [Formulate the point trajectory as combination of camera motion, global object motion, and local object motion.]
% [Discuss the simplification we can make to translate local object motion signal to point trajectories]
% [Refer to a later result figure to demonstrate the effectiveness of our design]
As we aim to utilize scene-space point trajectories to control object local motions, our focus lies on converting each scene-space control point $p_\text{scene}^l$ into its corresponding screen-space point $p_\text{screen}^l$. This involves transformations considering both camera and object global motion:
\begin{equation}
    p_\text{screen}^l = \mathcal{T}_\text{camera}^l(\mathcal{T}_\text{global}^l(p_\text{scene}^l)),
\end{equation}
where $\mathcal{T}_\text{global}^l(\cdot)$ represents object global motion transformation. Assuming negligible depth changes during local motion relative to global motion – a reasonable assumption as local motion often occurs within a similar depth plane (e.g., a waving hand) – we assign all local motion points the same depth as their initial positions. This simplifies the transformation to be based on camera motion. See Fig.~\ref{fig:xxx} and our supplementary documents for further details.


\subsection{Motion-conditioned Video Generation}
% [Discuss the role of video generation model. This plays the role of the synthesizing the final video content respecting all the conditions.]
% [Motivate the use of video diffusion model.]
% [Summarize the technical details of the video generation module: DiT backbone, incorporate trajectory based conditions and bounding-box conditions with separate conditioning mechanisms.]
Video diffusion models have emerged as the dominant paradigm for video generation.
We build our motion-conditioned video generation model upon a pre-trained Diffusion Transformer (DiT)-based (~\cite{peebles2023scalable}) image-to-video model.
This model is an internally-developed standard adaptation of DiT to support video generation, similar to existing open-source video DiT adaption such as~\cite{opensora} and ~\cite{yang2024cogvideox}.
We adapt the model to our motion-conditioned generation problem by fine-tuning it while incorporating the screen-space motion conditions: point trajectories and bounding-box sequence.

\input{Figures/fig-method-motion-conditioning}
% \paragraph{\textbf{Motion Signal Conditioning}}

\noindent\textbf{Point-Trajectory Conditioning.}
% [Discuss the representation of trajectory: encoding each trajectory into compact DCT representation.]
% [Describe the motivation for this representation. Insight: point tracking often has low temporal frequencies and therefore long trajectory can be represented with a few coefficients. DC component naturally encodes the position at the first frames, explicitly ground trajectory with location in the first frame. Advantages: each trajectory can be represented as a token and DCT serves as token embedding. Therefore, they can be seamlessly incorporated into DiT framework via in-context conditioning, this provides the simplicity for our framework. Another advantage is the efficiency in data organizing and loading, makes it possible to precompute trajectories and possible to handle different number of trajectories from very sparse to very dense.]
We represent $N$ point trajectories by encoding each into a compact set of Discrete Cosine Transform (DCT)~\cite{ahmed1974discrete} coefficients. Due to the low temporal frequency nature of point tracking, we can compress long trajectories into $K$ coefficients ($K=10$ is used for all experiments in this paper), with the DC component encoding the initial position, grounding the trajectory's start point explicitly. This compact representation, $C_\text{traj}\in\mathbb{R}^{N\times K \times 2}$, offers two important advantages. First, it simplifies and motion data handling, allows flexible handling of varying trajectory densities and improves efficiency through pre-computation. Second, integrates seamlessly into the DiT framework via in-context conditioning. Each trajectory is treated as an individual token, with its embedding derived from the DCT coefficients.


\noindent\textbf{Bbox-sequence Conditioning}
% [Discuss the rationale for representing bounding box separately from the trajectory: 1. Make explicitly the separation of camera and object motion, 2. Bounding-box object control can benefit from strong spatiotemporal injection.]
% [Discuss our design of bounding box conditioning: encode bounding-box sequence spatiotemporally into feature sequence. Use the pre-trained 3DVAE. Rasterize box into masks and encode in the input channels to 3DVAE.]
% [Explain the rationale of this way of encoding bounding boxes]
% [Discuss how the resulting box embedding are combined with the visual token embedding during DiT training.]
Bounding boxes convey complex spatial information (position, shape, pose) and are injected separately from trajectories to distinguish between camera and object global motion. 
We encode bbox sequences as spatio-temporal embeddings by first rasterizing them into unique color-coded masks, forming an RGB sequence $C_\text{bbox}^\text{RGB}\in \mathbb{R}^{L\times H\times W\times 3}$.
This sequence is then encoded into spatio-temporal embeddings $C_\text{bbox}\in \mathbb{R}^{L'\times H'\times W'\times C}$ using the same pre-trained video autoencoder (3D-VAE) from the base DiT model. These embeddings are patchified into tokens and added to the noisy video latent tokens, as illustrated in Fig.~\ref{fig:motion-conditioning}.

\subsubsection{Model Training}
% [Discuss the training procedure: provides the generic Diffusion Model training formulation. Modify the formulation to incorporate our conditioning signals.]
% [Mention that we also retain the text information. Explain the rationale for using text prompt: easier to fine tune from pretrained models, offers additional flexibility in controls. Mention that text prompt can either be user-provided, or automatically obtained during test time.]
% [Mention the chunk-based encoding scheme of our 3DVAE. Describe how that was adapted in our model design: this determines the lengths of the video we are modeling.]
% [Discuss the training details: how we define input and output, how we define the sampling percentage for each conditioning, the noise scheduling used during training, cfg details.]
% [Discuss the inference details: how many sampling steps, sampling strategy, cfg…]
Since we adopt a latent diffusion model, all RGB-space data are compressed into tokens within the latent space through a 3D-VAE encoder. The motion-conditioned model is optimized using the underlying flow-matching loss~\cite{lipmanflow,liu2023instaflow}. Specifically, denoting the ground-truth video latents as $X^1$ and noise as $X^0\sim\mathcal{N}(0,1)$, the noisy input is produced by linear interpolation $X^t=t X^1+(1-t)X^0$ at timestep $t$. The model $v_{\theta}$ predicts the velocity $V^t=\frac{d}{dt}X^t=X^1-X^0$. The training objective is:
\begin{equation}
    \mathcal{L} = \min _{\theta} \mathbb{E}_{t,X^0,X^1} \left[\Vert V^t -v_{\theta}(X^t,t \,|\, C_\text{img},C_\text{traj},C_\text{bbox},C_\text{txt})   \Vert_2^2 \right],
\end{equation}
where $C_\text{img}$, $C_\text{traj}$, $C_\text{bbox}$, $C_\text{txt}$ denote the input image, point trajectory, bbox, and text prompt, respectively.
Note that we also retain the text conditioning to offer additional flexibility in controlling video content changes. After training, the clean video latent tokens $\hat{X^1}$ can be generated conditioning on the input image, text prompt, and screen-space motion signals, which are then decoded back to RGB frames.


\subsection{Arbitrary-length Videos with Auto-regression}
% [Motivate the needs for modeling videos autoregressively: 1. Modeling arbitrarily long video at once is expensive, and constraining the applications to fixed-length videos. 2. In many scenarios motion signals are more naturally associated with shorter chunks, e.g. in designing cinematic shots people often design motion and blocking scenes for short period of time and piecing the key moments together.]
% [Discuss how our framework can be extended to handle long video sequence in autoregressive manner.]
% [Discuss the detail of our AR training method.]
% [Discuss how this can be applied during test time.]

Generating arbitrary-length videos is beneficial for cinematic storytelling. We achieve this through auto-regressive generation, which is more computationally efficient than modeling long videos directly and reflect the fact that complex video shots are often composed of a sequence of short, simple shots put together in sequence.
While our image-to-video framework naturally supports training-free long video generation in an auto-regressive manner due to it being I2V, we found that this often results in noticeable motion discontinuities, as a single conditional image lacks sufficient temporal motion information.
To address this, we train \MOCA$_\text{AR}$ with an additional conditioning on short video clips, $C_{vid}$ (16 frames). This overlapping short-clip strategy conditions each generation step on the previous spatiotemporal context, resulting in natural transitions. During inference, the model generates videos of arbitrary length with independent motion control per 
generation iteration. To further refine the input motion signals and align them with the training setup, we recompute the screen-space motion signals by combining the user’s intent with back-traced motions, including both bbox sequences and trajectories (detailed in the supplement). This approach ensures smoother and more consistent motion generation.

==> Sections/sec-4-applications-long.tex <==
\section{Applications}
\label{sec-4-applications}

\MOCA provides a solution for flexible controls of both camera and object motion in a scene-aware manner. This enables our main application of cinematic shot design framework, allowing users to interactively manage key motion aspects of a shot. 
Additionally, the flexibility of our motion representations makes it possible to naturally apply our framework on a variety of simple video-based editing tasks, including motion transfer and video-to-video transforms such as localized edit propagation (e.g., adding, removing, or replacing elements) and global appearance transform (e.g., style modifications).

\input{Figures/fig-app-shot-design}
\subsection{Shot Design with Joint Camera and Object Control}

Our shot design pipeline begins with an input image, where users specify 3D camera motion and object motion, and aligning them to a timeline. These user-defined intentions are transformed into screen-space conditioning signals, which are input into the video generation model. As illustrated in Fig.~\ref{fig:app-shot-design}, our framework enables precise and independent control of object and camera motion in a scene-aware manner, allowing for the design of highly dynamic and visually compelling shots while closely following the provided motion design. 

In Fig.~\ref{fig:app-shot-design}, it's worth noting that in both examples the results in each column follow the same camera motion while the object motions change according to the corresponding specified object controls. By placing the bounding box in a scene-aware manner, users can achieve various scene-space effect. For example, this makes it possible to induce the car in the bottom example to stay still (first row) or moving forward (second row) and backward (third row) on the road. Importantly, such scene-anchored motion is preserve while the camera motion change independently. This highlights the importance of scene-aware object motion controls.

\input{Figures/fig-app-shot-design-longvid}
\textbf{Long Videos with Complex Trajectories.}
To generate extended videos featuring complex camera and object motions, \MOCA employs a ``specification-generation'' loop. This approach allows users to define motion signals for each segment and subsequently generate video chunks in an auto-regressive manner. Inspired by animation workflows~\cite{xing2024tooncrafter,tang2025generativeaicelanimationsurvey}, \MOCA combines keyframing and interpolation to create intricate motion paths. Specifically, users can set keyframes for object and camera motions, and the system interpolates between these keyframes to produce smooth and coherent trajectories. 

As demonstrated in Fig.~\ref{fig:app-shot-design-longvid}, our method can generate long videos with complex sequence of camera motion controls. We showed two video results for each input image, resulting from the same camera controls (note that almost identical camera motion were generated for the two results) while intentionally using different object global motion control.

\input{Figures/fig-app-shot-design-local-motion}
\subsection{Object Local Motion Control.}

\MOCA also enables controlling local object motion to potentially support drag-based editing and generation. 
Users can define local object motions by directly specifying drag-based trajectories within the object's own coordinates. These point trajectories are then transformed to the appropriate screen-space point trajectories for conditioning the video generation model, taking into account both the camera and the object global motion. 
As illustrated in Fig.~\ref{fig:app-shot-design-local-motion}, our method can generate diverse and fine-grained local motions, making it possible to generate different variations of the object movements (\eg the different ways the arms of the baby move)

In addition, thanks to our dedicated motion translation module that accounts for the coordination between local motion and camera motion as well as global object motion,
consistent local object motion control can be achieved with different camera and object dynamics (bottom row of Fig.~\ref{fig:app-shot-design-local-motion}). This opens the possibility of incorporating local object motion control into the shot design framework described above.
%Our framework extends previous drag-based editing and generation approaches by incorporating local object motion control in a 3D-aware manner, surpassing the capabilities of prior works~\cite{pan2023drag,niu2025mofa}. While traditional drag-based methods permit manipulation of object trajectories in 2D space, our approach supports both drag-based and 3D-aware local object motion control, enabling users to create more sophisticated and spatially consistent motions.

\input{Figures/fig-additional-apps}
\subsection{Additional Applications: Simple Video-based Editing Tasks}

\textbf{Motion Transfer.}
Our method can be adapted to perform motion transfer from an input video to an input image that shares a structural similarity with the initial frames of the reference video. By leveraging the versatile screen-space conditioning representation, our framework effectively captures and transfers both object and camera motions, even for cases that involves 3D transform, without the need for explicit 3D camera pose extraction from the reference video. As shown in Fig.~\ref{fig:additional-apps}, a rotating movement of an apple was transferred to rotate the lion's head. 

\textbf{Video Editing.}
The concept of motion transfer can be extended to facilitate video editing, where the input image is derived from the first frame of the video through image editing~\cite{brooks2023instructpix2pix}. Utilizing the versatile screen-space conditioning representation, our method propagates extracted object and camera motions to the derived image, ensuring consistent and realistic dynamics, similar to~\cite{liu2024generative}. Fig.~\ref{fig:additional-apps} shows two examples where the edits performed on the initial frame of a video is propagated to results in a fully edited video, using the motion signals extracted from the original videos. 

==> Sections/sec-5-evaluation-old.tex <==

\section{Experiments}
\label{sec-5-evaluation}
\subsection{Implementation Details}
%data
\noindent\textbf{Data.} We collect $\sim$1.1M high-quality videos and extract the bounding boxes and sparse point tracking annotations using DEVA~\cite{cheng2023tracking} and RAFT~\cite{teed2020raft}. To ensure reliable motions, we filter videos using keyword-based criteria (e.g., $\texttt{vector}$, $\texttt{animation}$) and a threshold on valid tracking length. Bounding boxes are further filtered based on thresholds for adjacent-frame IoU, size change ratio, position change (Euclidean distance), and whether the object associated with the bounding box belongs to our interested moving object list. In the end, we obtained $\sim$600K videos with good motion quality and high-fidelity annotations. During training, with 80\% probability, we randomly select $N$ point trajectories, where $N \sim \mathcal{U}(0, 100)$. With 10\% probability, points are selected only from the moving object regions, and with another 10\% probability, points are selected from the non-moving object regions.

%% TODO: reason for this sampling
% model training
\noindent\textbf{Model.} Our \MOCA is fine-tuned based on a pre-trained image-to-video DiT model for 100K steps with a batch size of 256 using AdamW~\cite{loshchilov2017decoupled}, on the learning rate 1e-5 with a weight decay of 0.1. It is mainly trained on 32 and 64 frames with 12 and 24 FPS at a resolution of 640$\times$352. The results can be upscaled  to 720p using a super-resolution model. 
% TODO: model inference
During inference, we apply classifier-free guidance for text condition~\cite{ho2022classifier}.




\subsection{Camera Motion Control Quality}
To evaluate the quality of camera motion control, following~\cite{he2024cameractrl,wang2024motionctrl}, we employ rotation error (RotErr.), translation error (TransErr.), and CamMC as the metrics. Additionally, we compute Fr\'echet inception distance (FID)~\cite{heusel2017gans} to measure the quality and fidelity of the generated frames, and Fr\'echet Video Distance (FVD)~\cite{unterthiner2019fvd} to measure the temporal motion dynamics of the generated videos in both spatial and temporal domains. We compute these metrics on 1K videos randomly sampled from RealEstate-10K~\cite{zhou2018stereo} test set (@640$\times$352 with 14 frames).

We compare our method against two state-of-the-art camera-motion-controlled image-to-video methods: MotionCtrl~\cite{wang2024motionctrl} and CameraCtrl~\cite{he2024cameractrl}. The quantitative results are presented in Table~\ref{tab:quan_compare_camera}. It is worth noting that both MotionCtrl and CameraCtrl are trained on RealEstate10K train set, which provides them with a significant advantage on the in-domain test set.
Nevertheless, according to the results, our proposed method still outperforms previous approaches in all metrics under the zero-shot setting. 
%% Thanks to xxx, reason
The visual comparison is shown in Fig.~\ref{fig:eval-camera-control}, where the motion generated by MotionCtrl and CameraCtrl exhibits low quality, due to their necessity of training on video datasets (RealEstate10K) with 3D camera pose labels, which lacks diversity and contains only static estate scene. Additionally, our method supports controlling intrinsic parameters to produce more advanced cinematic shots like dolly zoom (see Fig.~\ref{fig:eval-camera-control}(right)).

%%%%%%%%%%% Figure: Evalulation -- Camera Control %%%%%%%%%%%%
\input{Figures/fig-eval-camera-control}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/tab-camera-motion}

% [Analyze the results.]
% [Refer to figure \ref{fig:eval-camera-control}. Discuss the ability of our method in handling the change in intrinsic as well as extrinsic camera parameters. Compare our methods and baselines for complex camera patterns such as Dolly-Zoom and Spiraling.]



\subsection{3D-Aware Object Motion Control Quality}
% To measure the object motion control performance, we adopt the Euclidean distance between the predicted~\cite{karaev2024cotracker3} and ground-truth object central trajectories (ObjMC)~\cite{wu2025draganything}. Additionally, we employ FID to compare the generated frame quality.
Following~\cite{wu2025draganything,wang2024motionctrl}, to measure the object motion control performance, we adopt ObjMC and FID as the metrics, and compute on
VIPSeg~\cite{miao2022large} filtered val set with 116 samples by excluding videos without moving object (@640$\times$352 with 14 frames). We compare our approach with DragAnything~\cite{wu2025draganything}, MOFA-Video~\cite{niu2025mofa}, and TrackDiffusion~\cite{li2023trackdiffusion}, and report the quantitative results in Table~\ref{tab:quan_compare_object}.
Our method demonstrates significant superiority over other baselines in both object control accuracy (ObjMC) and frame quality (FID), which is further evidenced in Fig.~\ref{fig:eval-object-control}. 
%% TODO: analysis a little bit...
%Emphasize that existing baseline cannot enable 3D-aware controls.]


%%%%%%%%%%% Figure: Evalulation -- Object Motion Control %%%%%%%%%%%%
\input{Figures/fig-eval-object-control}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/tab-object-global-motion}

% [Motivate the experiments. We want to evaluate whether our method can implement pure bounding-box based object motion controls without camera motion controls.]
% [Describe the evaluation protocol]
% [Describe the baseline methods]
% [Describe the evaluation metrics]

% [Analyze the results. Emphasize the fact that our method performs on par or better than others in bbox following. Also analyze the effectiveness of our bbox conditioning mechanism compared to baseline strategies.]

% [Refer to the figure \ref{fig:eval-object-control} and explain the results. Emphasize that existing baseline cannot enable 3D-aware controls.]

\subsection{Joint Camera and Object Control}
\input{Tables/tab-user-study}
%%%%%%%%%%% Figure: Evalulation -- Shot Design %%%%%%%%%%%%
\input{Figures/fig-eval-shot-design}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% [Focus directly on the task of joint camera and object control in 3D-Aware manner. For this we only need to compare to MotionCtrl and our adopted version of DragNUWA]

% [For this, we need to derive an evaluation protocol with a user study. Consider two versions for each baseline: 1. The original implementation, 2. Incorporating our motion signal synthesizer module.]

% [Discuss the user study results]

% [Refer to figure \ref{fig:eval-shot-design} and discuss the results]
% Table~\ref{tab:user_study}
We conducted a user study (detailed in the supplementary) to evaluate the perceptual quality of the joint camera and object motion control on real-case images in a 3D-scene-aware manner. We compare with drag-based I2V methods DragAnything~\cite{wu2025draganything} and MOFA-Video~\cite{niu2025mofa}. In addition to the point trajectory for object local motion control, we feed point trajectory from our depth-based warping and bbox sequence to them for camera and object global motion control. The participants were asked to choose the best result in terms of motion adherence, motion quality, and frame fidelity. The statistics from the responses of 35 participants are presented in Table~\ref{tab:user_study}. Our method demonstrates significant superiority over other competitors in all aspects. The visual results in Fig.~\ref{fig:eval-shot-design} xxx


\input{Figures/fig-eval-camera-ablation}
\subsection{Ablation Studies}
\input{Tables/tab-ablation-study}
\paragraph{\textbf{Camera Motion Representation.}} We construct the following baselines to investigate the effectiveness of our camera motion representation: Gaussian map: 2D gaussian blurred sparse optical-flow map, which is widely adopted~\cite{wang2024motionctrl,wu2025draganything,mou2024revideo}, Plucker embedding~\cite{he2024cameractrl,xu2024camco,bahmani2024vd3d}, and Trajectory coefficients (Ours). The quantitative comparison is tabulated in Table~\ref{tab:ablation_study_camera}. Noted that we plucker embedding variant necessitate training on video dataset with 3D camera pose labels, we select RealEstate10K training set following~\cite{wang2024motionctrl,he2024cameractrl}. Fig.~\ref{fig:eval-camera-ablation}.

\paragraph{\textbf{Bbox Conditioning.}}
We further evaluate the effectiveness of our bbox conditioning design. We apply the closed-source conditioning design from~\cite{wangboximator} to our base model, by concatenating bbox coordinates to visual tokens. The results in the last two columns in Table~\ref{tab:quan_compare_object} demonstrate the superiority of our color-coding map design.




